Agnostic Learning by Refuting

The sample complexity of learning a Boolean-valued function class is precisely characterized by its Rademacher complexity. This has little bearing, however, on the sample complexity of \emph{efficient} agnostic learning. We introduce \emph{refutation complexity}, a natural computational analog of Rademacher complexity of a Boolean concept class and show that it exactly characterizes the sample complexity of \emph{efficient} agnostic learning. Informally, refutation complexity of a class $\mathcal{C}$ is the minimum number of example-label pairs required to efficiently distinguish between the case that the labels correlate with the evaluation of some member of $\mathcal{C}$ (\emph{structure}) and the case where the labels are i.i.d. Rademacher random variables (\emph{noise}). The easy direction of this relationship was implicitly used in the recent framework for improper PAC learning lower bounds of Daniely and co-authors via connections to the hardness of refuting random constraint satisfaction problems. Our work can be seen as making the relationship between agnostic learning and refutation implicit in their work into an explicit equivalence. In a recent, independent work, Salil Vadhan discovered a similar relationship between refutation and PAC-learning in the realizable (i.e. noiseless) case.

==> content/abstract.tex <==
%!TEX root=../main.tex
The sample complexity of learning a Boolean-valued function class is precisely characterized by its Rademacher complexity. This has little bearing, however, on the sample complexity of \emph{efficient} agnostic learning. 

We introduce \emph{refutation complexity}, a natural computational analog of Rademacher complexity of a Boolean concept class and show that it exactly characterizes the sample complexity of \emph{efficient} agnostic learning. Informally, refutation complexity of a class $\C$ is the minimum number of  example-label pairs required to efficiently distinguish between the case that the labels correlate with the evaluation of some member of $\C$ (\emph{structure}) and the case where the labels are i.i.d. Rademacher random variables (\emph{noise}). The easy direction of this relationship was implicitly used in the recent framework for improper PAC learning lower bounds of Daniely and co-authors \cite{DBLP:conf/stoc/Daniely16,DBLP:conf/stoc/DanielyLS14,daniely2016complexity} via connections to the hardness of refuting random constraint satisfaction problems. Our work can be seen as making the relationship between agnostic learning and refutation implicit in their work into an explicit equivalence. 
In a recent, independent work, Salil Vadhan \cite{vadhan2017learning} discovered a similar relationship between refutation and PAC-learning in the realizable (i.e. noiseless) case. 





% We introduce \emph{refutation complexity}, a computational analog of the Rademacher complexity of a Boolean concept class $\C$ and show that it characterizes the complexity of efficient agnostic learning of $\C$ over a given distribution $\cD$ over examples. One direction of this relationship was implicitly used in the recent work of \cite{DBLP:conf/stoc/DanielyLS14} (and follow ups) to establish lower bounds on PAC learning various concept classes via a connection to the problem of refuting random CSPs. Our work can be seen as clarifying the relationship between learning and refutation and in particular establishing an equivalence between the two problems. 

==> content/intro.tex <==
%!TEX root=../main.tex
\section{Introduction}
Statistical complexity characterizes the information theoretic threshold for the amount of data required for any supervised learning task. However, the amount of data required for \emph{efficient} learning, whenever it is possible, can be significantly different from the statistical complexity.  For example, algorithms based on polynomial regression (\cite{DBLP:journals/siamcomp/KalaiKMS08,DBLP:conf/colt/KaneKM13,Klivans:2008:LGC:1470582.1470603}) guarantee efficient (improper, i.e. return a hypothesis not necessarily in the target class) learning while using data that is a polynomial factor larger than the statistical complexity. There is a systematic effort to study the trade-offs between computational and statistical complexity \cite{DBLP:journals/corr/abs-1304-0828,Chandrasekaran26032013} and a growing body of work has provided explicit examples \cite{DBLP:journals/siamcomp/DecaturGR99,DBLP:conf/nips/DanielyLS13,DBLP:journals/corr/BarakM15} of natural settings where efficient learning provably requires data that is at least a polynomial factor larger than the statistical complexity under some plausible complexity theoretic assumptions. 

In the light of the above work, we focus on obtaining a simple and useful characterization of the sample complexity of \emph{efficient} supervised learning. There's a simple and elegant characterization of the statistical complexity of learning in terms of the Rademacher complexity \footnote{The related notion of VC Dimension of $\C$ characterizes the data required to learn $\C$ over \emph{worst-case} distributions.}. In this note, we give a natural analog of Rademacher complexity that precisely characterizes the amount of data required for \emph{efficient agnostic} (i.e. noisy, see Definition \ref{def:agnostic-learning}) learning. 


% There's now a growing body of 
% Central to learning theory are the notions of statistical complexity that captures the amount of data required for learning (possibly inefficiently), and computational complexity that focuses on designing and analyzing efficient algorithms for learning. While there are a number of classical examples where efficient learning algorithms 


% While traditionally, these notions have been treated separately, there's now a growing body of work (\cite{DBLP:journals/corr/BarakM15},\FIXME), starting with the work of Daniely , that the amount of data required for efficient learning can differ drastically from the statistical complexity. 





% Starting with the work of Daniely \cite{DBLP:conf/nips/DanielyLS13}, there's a growing body of evidence (see \cite{DBLP:journals/corr/BarakM15}, that shows natural settings where one can design provable faster learning algorithms by using significantly more data than the statistical complexity. There are natural instances where this trade-off between computational and statistical complexities can lead to dramatic effects. For example, the computational complexity of predicting $n$ dimensional, rank $r$ third order tensors drops from super-polynomial to polynomial by blowing up the number of samples by a factor of $\sqrt{n}.$ 


 % can under plausible complexity theoretic assumptions),influential recent works \cite{DBLP:journals/corr/BarakM15}, have revealed
{}


% An early achievement of learning theory precisely characterizes the amount of data required to learn any concept class $\C$ over a given distribution $\cD$ over its domain in terms of the Rademacher Complexity \footnote{The related notion of VC Dimension of $\C$ characterizes the data required to learn $\C$ over \emph{worst-case} distributions}. In this note, we give a natural analog that precisely characterizes the amount of data required for 

% {}



% {}

For a class $\C$ of concepts on $\R^n$, any distribution $\cD$ on $\R^n$, the \emph{Rademacher Complexity} of $\C$, $\cR_m(\C)$ is the following quantity: 
\begin{align}
\mathcal{R}_m(\C) = \E_{\begin{subarray}{c} x_i \sim_{i.i.d.} \cD\\ 1\leq i \leq m \end{subarray}}\left[\E_{\begin{subarray}{c}\sigma_i \sim_{i.i.d.} \{\pm 1\} \\ 1 \leq i \leq m \end{subarray} }\left[\frac{1}{m}\sup_{c\in \C}\sum_{i=1}^m  \sigma_{i}c(x_i)\right]\right].
\end{align}
Classical results \cite{BartlettM02} establish that $\cR_m(\C) = \epsilon$ if and only if there's an algorithm to learn $\C$ over $\cD$ with error at most $\epsilon$ with $\Theta(m)$ samples, thus characterizing the sample-complexity of $\epsilon$-error agnostic learning. % In particular, the least $m$ such that $\cR_m(\C) < \epsilon$, characterizes up to constant factors, the sample complexity of agnostically learning $\C$ (by a possibly inefficient algorithm) with respect to $\cD$ with any constant error.  %In particular, agnostically learning a concept class to a vanishing error requires $m$ samples where $m(n)$ satisfies $\cR_m(\C) = o(1)$ 

% Designing supervised learning algorithms has been traditionally broken down into a statistical component: bounding the sample complexity and an algorithmic component: showing an efficient learning algorithm. The statistical learning complexity of a class is the minimum number of samples that makes some (possibly inefficient) learning algorithm for the class succeed. For Boolean concepts (i.e., functions that output either $0$ or $1$), this is entirely characterized by elegant classical notions such as VC dimension \cite{vapnik1971uniform} and the Rademacher complexity of the class \cite{BartlettM02}. 


%  Traditionally, supervised learning is dichotomized into \emph{Statistical Learning Theory} and \emph{Computational Learning Theory}. While the first is concerned with establishing sample complexity bounds: namely, analysing the number of samples required to correctly choose an underlying, unknown target concept, the second is concerned with the algorithmic aspects and the complexity of computing the aforementioned target concept.	
 
% For Boolean concepts the statistical complexity is a well understood problem and is governed by magnitudes such as \emph{VC dimension} \cite{vapnik1971uniform} or \emph{Rademacher Complexity} of the class to be learnt \cite{ BartlettM02}. The Rademacher complexity of a class $\C$ measures how much a concept may be correlated with purely random bits over an empirical sample set. Namely, we let $\D^{\otimes m}$ be a distribution over $m$ i.i.d samples drawn according to distribution $\D$ and $\U_m$ be a uniform distribution over $m$ i.i.d random bits (Rademacher variables). Then the Rademacher complexity of a class $\C$ w.r.t $\D$ is defined as
% \begin{align}
% \mathcal{R}_m(\C) = \E_{x_1,\ldots,x_m \sim D^{\otimes m}}\left[\E_{\sigma_1,\ldots,\sigma_m \sim \U_m}\left[\frac{1}{m}\sup_{c\in \C}\sum_{i=1}^m  \sigma_{i}c(x_i)\right]\right]
% \end{align}
% A classical result in Statistical Learning \cite{BartlettM02} states that the Rademacher complexity completely governs the number of samples needed in order to learn a boolean class. Specifically, to choose a concept $c\in \C$ whose accuracy is roughly of order $\epsilon$ the sample size needed is $m$ such that $\mathcal{R}_m(\C)< \epsilon$. Thus a class is learnable if and only if $\mathcal{R}_m(\C)$ tends to zero as $m$ grows.



% Understanding the computational complexity of learning  is a much more delicate problem, and has been the focal point of study for many research papers ever since the seminal work of Valiant \cite{valiant84}-- some are designed to produce new, non--trivial, learning algorithms while others are producing new lower bounds demonstrating the hardness of various learning problems (e.g. \cite{DBLP:journals/jacm/KearnsV94, Klivans09, daniely2014average, daniely2016complexity}). 

% Overall there are wide gaps between computational vs statistical learning thresholds for natural learning problems, and even simplest classes with small Rademacher complexity may require much more samples then needed from a statistical viewpoint. These wide gaps continue to hold even in the simplest of situations (such as agnostically learning Boolean monomials \cite{}.) 


%Traditionally, designing supervised learning algorithms is seen as composed of two atomic steps. The first, called as establishing ``identifiability'' or ``information theoretic threshold'' shows that there's a not too large upper bound on the number of samples required to uniquely determine the underlying, unknown target concept. In case of Boolean concepts, identiability is equivalent to establishing an upper bound on the Rademacher complexity or VC dimension. The Rademacher complexity of a class $\C$ of Boolean concepts on a distribution $\D$ on inputs equals $\E_{(x_1, x_2, \ldots, x_m) \sim \D^{\otimes m}} \E_{ (\sigma_1, \sigma_2, \ldots, \sigma_m) \sim \on^m} [ \sum_{ i = 1}^m c(x_i) \sigma_i]$ - the expected supremum of the correlation between completely random bits  (Rademacher variables) and the output of a single concept $c$ on i.i.d sample of size $m$ drawn according to $\D$. Informally, this quantity measures the maximum correlation that any member of $\C$ has with purely random bits (noise) when evaluated at a $m$-size sample chosen i.i.d. from $\D$. %The sample complexity of the algorithm, via a classical elegant argument can be chosen to be equal to the Rademacher complexity

%In most situations, the estimating a good upper bound on the Rademacher complexity of the underlying class $\C$ is easy and gets little elaboration. Indeed, for finite classes, a simple upper bound is just $\tilde{O}(\sqrt{m} \sqrt{ \log{|\C|}})$ which is enough to show that a information theoretic threshold for learning $\C$ is no more than $\tilde{O}(\log{(|\C|)})$ samples. The second step is the design of an (efficient) learning algorithm which usually involves creativity and is less amenable to a single general trick as above. 

In this note, we propose a natural computational analog of Rademacher complexity, called as the \emph{Refutation complexity} and show that it exactly determines the sample complexity of efficient agnostic learning. Given random labeled examples $\{(x_i, y_i)\}_{i \leq m}$ where $x_i$s are chosen i.i.d. according to $\cD$, we define the problem of \emph{refutation} as the task of distinguishing between the following two cases:
\begin{enumerate}[(a)]
 \item \textbf{Structure: } $\{(x_i,y_i)\}_{i \leq m}$ are i.i.d. from some distribution $\cD'$ with marginal on $x_i$s being $\cD$ and $\E_{(x,y) \sim \cD'}[c(x)y] = \Omega(1).$ That is, the given example-label pairs come from a distribution that correlates with some $c\in \C$, and 
 \item \textbf{Noise: }$y_i$s are uniform and independent Rademacher random variables. \label{s}
 \end{enumerate}
We define refutation complexity of $\C$ with respect to the distribution $\cD$ at a running time of $T(n)$ as the smallest $m$ for which there's a $T(n)$-time test for distinguishing between structure and noise cases above. 

To motivate this definition, observe that we can interpret the statistical complexity (via the connection to Rademacher complexity outlined above) of $\C$ over $\cD$ as the smallest $m$ for which no concept in $\C$ correlates with purely random noise (the i.i.d. draws from $\{ \pm 1\}.$) Thus, if the Rademacher complexity of $\C$ on $\cD$ with $m$ samples is small enough, then, given random labeled examples $\{ (x_i, y_i)\}_{i \leq m}$, we can (via an inefficient procedure) distinguish between the above two cases by computing the largest correlation of any $c \in \C$ when evaluated at $x_i$s with the $y_i$s. Thus, we can equivalently define statistical complexity as the smallest $m$ for which the above structure vs noise test succeeds. Thus, refutation complexity can be seen as a computational analog of Rademacher complexity. 

The main result of this note is the following theorem:
\begin{theorem}[ Refutation Complexity = Agnostic Learning Complexity, Informal] \label{thm:main-informal}
$\C$ has an efficient agnostic learning algorithm over a distribution $\cD$ with $m$ samples if and only if the refutation complexity of $\C$ at some polynomial running time is at most $O(m).$ 
\end{theorem}

\subsection{Comparison with \cite{vadhan2017learning}} 

In a recent, independent work, Vadhan \cite{vadhan2017learning} used similar arguments to establish a similar equivalence to Theorem \ref{thm:main-informal} between \emph{distribution independent PAC learning} in the realizable case (i.e. when the labels perfectly correlate with some concept in the target class) and a slightly different notion of refutation. In this notion, the refutation algorithm is required to distinguish the case that the sample that realizable (i.e., the labels agree with some concept from the class) from the case that the labels in the sample are i.i.d. Rademacher random variables.

Since agnostic learning is provably different from realizable PAC learning in general, the notions of refutation that characterize the  complexity of learning in the two models have to be necessarily different. Another interesting point of difference is that our equivalence is \emph{distribution-specific} and thus slightly more fine-grained in that it allows relating learnability on a given distribution to refutation on the same distribution. In contrast, Vadhan's characterization holds for distribution independent PAC learning. This difference arises entirely due to the the difference in the black-box boosting algorithms one can use in PAC vs agnostic settings\footnote{We thank Salil Vadhan for pointing this out to us.}: in the PAC learning case, the boosting algorithms modify the distribution of examples over the course of the execution and thus the characterization holds only in a distribution independent setting. In the agnostic setting, there are distribution specific boosting algorithms (such as that of \cite{DBLP:conf/nips/KalaiK09,feldman2010distribution}) that work by changing only the distributions of the labels while keeping the distribution of the example points unchanged. It is an interesting direction to investigate notions of refutation that allow \emph{distribution-specific} characterization of PAC learning in realizable case.

It's interesting to note how slight changes to in the formulation of the refutation problem changes the model of learning that it characterizes.

 % Despite the similarity to the proof technique in \cite{vadhan2017learning}, we believe that it's conceptually interesting to understand how different notions of refutation characterize the learning complexity in different learning models.

\subsection{Discussion}
\paragraph{Proper vs Improper Learning and the Framework of \cite{daniely2014average}} The agnostic learning algorithm we obtain using a refutation algorithm is \emph{improper} - that is, it doesn't necessarily produce a hypothesis from the class $\C$. This is not accidental - it's well known that the flexibility of \emph{improper} learning allows circumventing computational hardness results that afflict \emph{proper} learning. A simple example is the class of 3-term DNF formulas in $n$ variables: unless RP = NP, there's no polynomial time \emph{proper} learning algorithm for this class \cite{DBLP:journals/jacm/PittV88}, however, there's a simple $\poly(n,1/\epsilon)$-time \emph{improper} learning algorithm for it (for a discussion see, \cite{DBLP:journals/jmlr/Shalev-ShwartzST12}). On the flip side, the power of \emph{improper} learning makes the task of proving lower bound against such algorithms harder. The equivalence between refutation and agnostic learning holds for all (and thus, also improper) learning algorithms and thus can serve as a useful handle in understanding the complexity of improper learning.

Indeed this connection and in particular, the implication that learning implies refutation is implicit in the influential work of Daniely and co-authors \cite{DBLP:conf/stoc/Daniely16,daniely2016complexity,DBLP:conf/stoc/DanielyLS14} who showed (in the language of this paper) that a refutation algorithm for the concept classes of halfspaces and DNF formulas can be used to refute certain random constraint satisfaction problems \cite{MR3473335-Allen15,MR2121179-Feige02}. These works used such a reduction along with standard hardness assumptions for refuting random CSPs to obtain the first hardness results for improper PAC learning for the above classes. 

Our equivalence establishes the converse of the connection in these works and makes the connection between refutation and agnostic learning explicit. While a priori, it might appear that refutation (which asks for distinguishing between a pure noise in the labels from a correlated set of labels) is easier than agnostic learning, this work shows that any lower bound on (improper) learning has to necessarily be a lower bound for an associated refutation problem. Thus, to an extent, it shows that the above framework for improper agnostic learning lower bounds is essentially complete. 




%  it's conceptually important to understand the right notions of the refutation problem that characterize realizable (i.e. noiseless) PAC learning vs agnostic (i.e. with adversarial noise) learning. 




% Apart from the difference between the learning models characterized, this work has another interesting point of difference compared to Vadhan's \cite{vadhan2017learning}. First, the characterization 
% Technically, our equivalence result differs from that in 


% two observations are worth noting. First, our characterization is . This is 


\paragraph{Connections to Boosting/Property Testing} It is also illuminating to view the equivalence we show as saying that an oracle for refutation is sufficient for agnostic learning. This naturally leads to the question of what kind of oracle access to $\C$ is sufficient for (agnostic) learning. We discuss two natural oracles here: a weak-learning oracle and a property-testing oracle.

Known boosting (see \cite{freund1995desicion, schapire90}, \cite{DBLP:conf/nips/KalaiK09, feldman2010distribution}) algorithms imply that a \emph{weak-learning oracle} is sufficient for agnostically learning of $\C$. A weak learning oracle takes random example-label pairs and returns a hypothesis whose correlation with the labels from the input distribution is at least an inverse polynomial fraction of the correlation of the best-fitting hypothesis from $\C$. In learning literature, this is sometimes referred to as a \emph{weak-optimization} oracle for $\C$ - in that, it gives a inverse polynomial (potentially improperly) approximation to the correlation of the best fitting hypothesis from $\C$. It is not hard to see that such an oracle is enough to solve the refutation problem and thus is a potentially stronger access to $\C$ than the refutation algorithm. 

Our result implies that an much weaker algorithm is enough to get an agnostic learning algorithm - the refutation oracle doesn't return any hypothesis, it ``merely'' distinguishes between the case that the labels are completely random and independent of the examples from the case that the labels come from some distribution that correlates with some concept in $\C$. 

It is also instructive to compare a refutation oracle (or a ``structure`` vs ''noise'' tester) for $\C$ with a ``property-tester'' for $\C$. An $\alpha$-approximate property-testing algorithm for $\C$ uses random example-label pairs \footnote{Property testers are usually defined with $\alpha = 1$ and are in general also allowed to use membership queries. We use a definition that is similar in spirit but is more relevant for the comparison here.} from some distribution and accepts if the labels achieve a correlation of at least $\alpha$ with $\C$ and rejects if tevery $c \in \C$ has a correlation of at most $\alpha-\epsilon$ with the labels. We can interpret a property tester, thus, as a variant of the refutation oracle that must treat a distribution on example-label pairs that has a correlation of at most $\alpha-\epsilon$ with every $c \in \C$ as ``noise.'' In particular, the notion of what is ``unstructured/noise'' for a property tester is more stringent compared to a refutation algorithm. Indeed, this is not surprising: while testing is known to be no harder than \emph{proper} learning, it can be harder than \emph{improper} learning for some concept classes, once again illustrating the difference between proper and improper learning \cite{DBLP:journals/jacm/GoldreichGR98}. 

\paragraph{Using Refutation to get Learning Algorithms} It will be extremely interesting to understand if the equivalence between refutation and learning allows an application in the direction opposite to the one employed in the work of Daniely and co-authors and get new algorithms for agnostic learning. This is perhaps not too optimistic. The works of Daniely and co-authors establish a natural connection between the refutation problem for a concept class and refuting random CSPs. There are known algorithms for refuting random CSPs (see for e.g. \cite{DBLP:journals/corr/RaghavendraRS16,DBLP:conf/focs/Feige07,MR3473335-Allen15}) that use techniques that appear different from the usual tool-kit in agnostic learning (for e.g. the use of semi-definite programming) that might prove useful in obtaining new agnostic learning algorithms by building the required refutation algorithms. 
% In particular, taking $m$ samples $x_1, x_2, \ldots, x_m$ and computing the largest correlation of any $c \in \C$ evaluated at $x_i$s with i.i.d. Rademacher variables gives an (inefficient) test to distinguish between the cases when 1) labels that correlate with some function in $\C$ and computing the maximum correlation of an  Our computational analog will work with the smallest $m$ for which


% In a nutshell, the Refutation complexity of a class is defined to be as the least number of labeled examples needed, so that an efficient algorithm will distinguish between:

% \begin{enumerate}[(a)]
% \item\label{c} Labeled examples $(x_1,\sigma_1),\ldots, (x_1,\sigma_m)$  such that: $ \sup_{c\in \C}\frac{1}{m} \sum \sigma_i c(x_i) = \Omega(1)$.
% \item\label{s} Labeled examples $(x_1,\sigma_1),\ldots, (x_m,\sigma_m)$ such that $\sigma_i$ are completely random bits independent of $x$'s
% \end{enumerate}

 
%  To compare Refutation complexity to Rademacher complexity we first observe that if a class does not have vanishing Rademacher complexity, \ref{c} and \ref{s} may become indistinguishable as they might intersect. Next, we observe the following. Suppose we are given a sequence of labeled pairs $S= \{(x_1\sigma_1),\ldots, (x_m,\sigma_m)\}$ and we want to distinguish between the two cases \ref{c} and \ref{s}. Let us write for a fixed sample $S$:
%   \begin{align*}\mathcal{R}_m(\C,S) = \left[\frac{1}{m} \sup_{c\in \C} \sum_{i=1}^m \sigma_i c(x_i)\right] \end{align*}
%  One can show that if the class $\C$ is learnable, we can (w.h.p) distinguish between purely random bits and structured labels by computing $\mathcal{R}_m(\C,S)$ for sufficiently large $m$. Indeed, as discussed, learnability implies that if \ref{s} holds then $\E\left[\mathcal{R}_m(\C,S)\right]$ is sufficiently small for large enough $m$. In contrast we are guaranteed that $\mathcal{R}_m(\C,S)$ will be bounded away from $0$ if \ref{c} holds.
 
% To summarize, we can interpret the Rademacher complexity as an inefficient distinguisher between purely random bits and bits that correlate with concept from the class, and a class is learnable if and only if there is an inefficient distinguisher between \ref{c} and \ref{s} in the form of the Rademacher statistic $\mathcal{R}_m (\C,S)$.


 
 % The notion of Refutation complexity, demands that we hold an \emph{efficient} distinguisher between \ref{c} and \ref{s}, thus it can be interpreted as an effective analogue of the Rademacher notion. In turn, our main result states that the class can be learnt at time that scales polynomially with the refutation complexity.

% It is also informative to compare our result to Boosting \cite{freund1995desicion}. A boosting meta--algorithm learns a target concept class using access to a \emph{weak learner oracle}--that outputs a slightly better then random hypothesis for a given distribution. The underlying theorem for Boosting \cite{freund1995desicion, schapire90} shows that given access to a weak learning oracle, one can efficiently learn the class. These results have been extended to the Agnostic setting in the works of \cite{DBLP:conf/nips/KalaiK09, feldman2010distribution}.

% A weak learning oracle can be easily turned to a refutation algorithm. Indeed, a hypothesis that does slightly better then random guessing exists only if \ref{c} holds and serves as a proof that the labelings are not completely random. Hence we can distinguish between \ref{c} and \ref{s} by running a weak learner oracle and check if it succeeds. Boosting theorem then states that a class is efficiently learnable if there exists such an efficient distinguisher that outputs a slightly better then random guessing.

% Our result states that an even weaker oracle then the standard boosting oracle is needed for learning. While a weak learning oracle returns a weak hypothesis, the oracle we consider merely decides if such a hypothesis exists -- without necessarily providing the aforementioned hypothesis.

% The connection between learning and refutation is implicitly present in the works \cite{DBLP:conf/stoc/DanielyLS14, DBLP:conf/stoc/Daniely16}. These recent works suggested new proof techniques to derive hardness for learning under certain hardness assumptions for refuting constraint satisfaction problems. Building upon these works \cite{daniely2016complexity, DBLP:conf/stoc/Daniely16} were able to prove hardness results for learning DNF and agnostic half spaces, based upon a generalization of Feige's conjecture about hardness of refuting random $3$-SAT \cite{DBLP:conf/coco/Feige02}.  

% Thus, while lower bounding the refutation complexity serves as a tool to show hardness of learning, our work shows that the connection goes in the other direction too. While a priori, the approach of Daniely could look surprising from a learning theory perspective, our result thus establishes that the approach of Daniely is in fact quite natural in the context of showing (improper) learning lower bounds.

% In a recent and independent work \cite{vadhan2017learning} achieved a result similar to ours in a the realizable, distribution independent setting. Salil showed an equivalence between PAC (reaalizable) efficient learnability of a class $\C$ and refutation of a system of equations with random-right-hand-side bits (where satisfaction of the equations proves that the class is realizable).

%  Our work differs in two aspects. 
% \begin{enumerate}
% \item We describe agnostic learning where Salil's paper describes PAC learning in the realizable sense. In turn, the algorithm needs to identify \emph{any} sequence that is correlated with the any possible labelings in the hypothesis class (and not just realizable) \rl{Is our definition more natural in the context of pseudorandomness?}
% \item Our results are distribution dependent. Thus, we require for the refutation algorithm, to distinguish under a fixed given distribution over $(x,y)\sim D$ pairs, and we achieve a distribution dependent characterization of learning.
% \end{enumerate}

% Remarkably, the techniques are very similar. Our proof first rely on the Boosting principle which allows converting weak learners into strong learners. Since we want to achieve guarantees for the agnostic setting, we rely here on an agnostic version of boosting due to \cite{DBLP:conf/nips/KalaiK09} (although, other existing agnostic  boosting methods can be readily applied, see \cite{feldman2010distribution}). The second tool in our arsenal is also apparent in Salil's work and we rely on a hybrid argument to construct a weak prediction algorithm from a refutation algorithm, following similar techniques to Yao's equivalence between pseudorandomness and next--bit unpredictability \cite{DBLP:conf/focs/Yao82a}.
\subsection{Proof Overview}
It is easy to see that efficient learning implies efficient refutation. For the other direction, we give an explicit, efficient algorithm that invokes the refutation algorithm a small number of times to get an agnostic learner for the class $\C$. This algorithm works in two steps - in the first step, it uses a refutation algorithm to come up with a \emph{weak-agnostic} learner: i.e. a hypothesis that achieves a correlation with the labels that is some tiny fraction of the correlation of the best hypothesis from $\C$. In the second step, it combined an off-the-shelf boosting algorithm with the weak learner above to get an agnostic learner with small error. 

The key idea in the transformation of a refutation algorithm into a weak-learner is to view the black-box refutation algorithm as a ``code'' for computing a function by manipulating the example-label pairs that it takes as input. A simple hybrid argument then shows that there's a small list of hypotheses generated by manipulating the inputs to the refutation algorithm that contains a good weak learner. We can find the best weak learner from the list by evaluating the error of each of the hypotheses in the list over a fresh batch of samples from the underlying distribution.
\subsection{Preliminaries}
We use $\U_m$ to denote the uniform distribution over $\on^m$ for any $m \in \N.$ 
We define agnostic learning here.
\begin{definition}[Agnostic Learning with respect to a distribution $\cD$] \label{def:agnostic-learning}
Let $\C$ be a class of Boolean concepts $\C \subseteq \{ f: \on^n \rightarrow \on \}$. $\C$ is said to be $\epsilon$-agnostically learnable in time $T(n,1/\epsilon)$ and samples $S(n,1/\epsilon)$ if there's an algorithm $\cA$ running in time $T(n,1/\epsilon)$ that takes $S(n,1/\epsilon)$ random labeled examples $\{ (x_i,y_i) \mid 1 \leq i \leq m\}$ where $(x_i,y_i)$s are i.i.d. from $\cD'$, such that the marginal on $x_i$ is $\cD$ and outputs with probability at least $3/4$, a hypothesis $h: \on^n \rightarrow \on$ such that $\E_{(x,y) \sim \cD'}\left[ \one{h(x)\ne y}\right] \leq \inf_{c \in \C} \E_{(x,y) \sim \cD'}\left[\one{c(x)\ne y}\right] + \epsilon.$ 
\end{definition}

% \begin{remark}
% In order to avoid notational clutter, we set $\epsilon$ to be some fixed quantity $\epsilon_0$ assumed to be some inverse polynomial. We do not state explicitly the dependence on $1/\epsilon_0$ so long as it is some fixed polynomial. 
% \end{remark}
% Specifically, they define an (α, γ)-weak agnostic learner to be a learning algorithm that produces a
% hypothesis with the error of at most 1/2 − γ whenever ∆ ≤ 1/2 − α.


% A $(\alpha, \gamma)$-weak agnostic learner for a class $\C$ of concepts on $\on^n$ with respect to a distribution $\cD$ is an algorithm that takes input i.i.d. sample $(x_1,y_1), (x_2, y_2), \ldots, (x_m,y_m)$ from a distribution $\cD'$ on $\on^n \rightarrow \on$ such that the marginal on $x_i$ is $\cD$ and with probability at least $3/4$ outputs a hypothesis $h$ such that $\E_{(x_i,y_i) \sim \cD'}[ h(x_i) y_i] \geq 2 \gamma$ whenever $\sup_{c \in \C} \E_{(x_i,y_i) \sim \cD'}[ c(x_i) y_i] > 2\alpha.$  







==> content/learning.tex <==
%!TEX root=../main.tex

\section{Refutation Complexity}
In this section, we define refutation complexity of a class of hypothesis with respect to a distribution $\cD$.
% In this section, we define refutation complexity: the algorithmic analog of Rademacher complexity. Readers familiar with the problem of refuting (or certifying) unsatisfiability of random constraint satisfaction problems will immediately see the similiarity in the notion. Indeed, one of the points we want to stress is to think of the refutation problem in the context of CSPs also as a computationally bounded analog of the problem of certifying "randomness" (which in the present case corresponds to having a small value for CSPs.)
% \Pnote{ this is somewhat rambling at this point and should be cleaned up. Also should be moved to the intro} 
% \Pnote{We start by defining a refutation algorithm for a class of Boolean functions $\C$. Informally, such an algorithm takes some example-label pairs and must distinguish whether the labels are ``structured'' (correlated with the evaluation of some function from the class) or are i.i.d. uniform over $\on$. It is instructive to compare this to a \emph{property testing} algorithm for $\C$. Such an algorithm is similar in the sense that it must take example-label pairs (a property tester is allows access to membership queries, but here, for comparison, we restrict to a tester that works with i.i.d. samples according to some distribution) but differs in the guarantees it offers where it must correctly (whp) decide if the labelling function is within $\C$ or $\epsilon$-far from $\C$. We can think of this as a more stringent version of refutation where a labeling function is structured only if it is contained in $\C$ and is considered ``noise'' if it is a tiny bit far from every function in $\C$. If we consider what labeling functions the algorithms must reject, then a property tester requires stronger guarantees and indeed, it's been known (cite Goldreich) that property tester could in fact be stronger than a learning algorithm. A refutation algorithm can be thought of as an extremely weak property tester which is required to reject only if the labeling function is completely random. Perhaps surprisingly, such an algorithm is enough to get an agnostic learning algorithm for the class $\C$.}




\begin{definition}[Refutation Algorithm for Distribution $\cD$]
Let $\C \subseteq \{f: \R^n \rightarrow \on\}$ be a class of Boolean concepts. Let $\cD$ be a distribution on $\R^n.$
% Let $\cD$ be a distribution on $\on^n.$

A $\delta$-\emph{refutation} algorithm $\cA$ for $\C$ on $\cD$ with $m = m(n)$ samples is a (possibly randomized) algorithm that takes input an $m$-tuple of points $\{ x_1, x_2, \ldots, x_m \} \subseteq \on^n$ and an $m$-tuple of labels $(\sigma_1, \sigma_2, \ldots, \sigma_m) \in \on^m$ and outputs either $\noise$ or $\unclear$ with the following guarantees:
\begin{enumerate}
\item \textbf{Completeness: } If $\{(x_i, \sigma_i)\}_{i \leq m}$ are i.i.d. from a distribution $\cD'$ on $\R^n \otimes \{\pm 1\}$ such that the marginal on $\R^n$ equals $\cD$ and $ \sup_{c \in \C} \E_{(x,\sigma) \sim \cD'}[c(x) \sigma] \geq \delta$, then, 
\[
\Pr_{\begin{subarray}{c}
\{(x_i,y_i)\}_{i \leq m} \sim_{i.i.d.} \cD'\\
 \text{ internal randomness of } \cA \end{subarray}} [ \text{ output = } \unclear] \geq 2/3.
\]
\item \textbf{ Soundness: } 
\[
\Pr_{\begin{subarray}{c}
(\sigma_1, \sigma_2, \ldots, \sigma_m) \sim \U_m\\
x_1,x_2, \ldots, x_m \sim \cD\\
 \text{ internal randomness of } \cA \end{subarray}} \Pr_{ } [ \text{ output = } \noise] \geq 2/3.
 \] 
\end{enumerate}
\end{definition}


\begin{definition}[$\delta$-Refutation Complexity]
Let $\C \subseteq \{f: \on^n \rightarrow \on\}$ be a class of Boolean concepts. 
Let $\cD$ be a distribution on $\on^n.$


The $\delta$-\emph{refutation complexity} of $\C$ on a distribution $\cD$ with running time $T(n)$ denoted by $\cR_{T(n),\delta}(\C)$, is the smallest $m = m(n,\delta)$ such that there exists a $\delta$-refutation algorithm for $\C$ on $\cD$ running in time $T(n)$ and $m$-samples. When $T(n)$ is not stated explicitly, we assume $T(n) = \poly(n)$ for some fixed polynomial in $n$. 
\end{definition}
\begin{remark}
Observe that the refutation complexity, just as Rademacher complexity is distribution dependent. Further, for $T(n) = \infty$, $\delta$-refutation complexity degenerates into Rademacher complexity. At non-trivially bounded running times (of special interest, of course, is polynomial time algorithms), refutation complexity captures the sample complexity of \emph{efficient} agnostic, improper learning $\C$ over $\cD$ as we show next and thus can be much larger than the Rademacher complexity.
\end{remark}

\section{Learning vs Refutation Complexity}

In this section, we establish the equivalence between agnostic learning a class $\C$ over a given distribution $\cD$ and the refutation problem with  respect to the distribution $\cD$ for the concept class $\C$.

We begin by showing the Learning implies Refutation, which is the easy direction.

\begin{lemma}[Learning implies Refutation]
Suppose $\C$ is $\epsilon$-agnostically learnable in time $T(n,\epsilon)$ and samples $S(n,\epsilon)$ over the distribution $\cD$.
% for an error parameter $\epsilon_0/4$.
Then, the refutation complexity of $\C$ with respect to the distribution $\cD$ at the running time $T(n,\delta/4)$ is at most $2S(n,\delta/4) + 128/\delta^2.$
\end{lemma}
\begin{proof}
Let $m = S(n,\delta/4) + 64/\delta^2.$ 

The $\delta$-refutation algorithm gets input $x_1, x_2, \ldots, x_{2m}$ and $\sigma_1, \sigma_2, \ldots, \sigma_{2m}.$ It runs the $\epsilon$-agnostic learner on examples $\{(x_i, \sigma_i)\}_{i =1}^m$ for $\epsilon = \delta/4$ and obtains a hypothesis $h$. Let $\cor_h = \frac{1}{m}\sum_{i =m+1}^{2m} \sigma_i \cdot h(x_i).$ If $\cor_h \geq \delta/2$, output $\unclear$ otherwise output $\noise.$

We now analyze the completeness and the soundness properties of this algorithm. 

First, suppose $\{(x_i, \sigma_i)\}_{i \leq 2m}$ were i.i.d. according to some $\cD'$ such that the marginal on $\R^n$ equals $\cD$. Let $\cor_f(\cD') = \E_{(x,y) \sim \cD'}[ f(x) y].$ Then, with probability $2/3$ over the draw of the sample, the agnostic learner produces a hypothesis $h$ such that $\cor_h \geq \cor_h(\cD') - \epsilon \geq \cor_c(\cD')-2\epsilon$ for every $c \in \C$. Thus, if $\cor_c(\cD') \geq \delta$, then, $\cor_h \geq \delta - \epsilon/2 \geq \delta/2.$ Thus, in this case, the algorithm above outputs $\unclear$ as desired.

Now suppose $\sigma_i$s are i.i.d. Rademacher and independent of $x_i$s. Then, since $\sigma_{m+1}, \ldots, \sim_{2m}$ are independent of $\sigma_1, \ldots, \sigma_m$, $\cor_h \leq \frac{4}{\sqrt{m}} < \delta/2$ using that $m  > 64/\delta^2.$

% The input to the refutation algorithm is a i.i.d. draw of $(x_1, x_2,\ldots, x_{2m})$ for $m = S(n)$ and a sequence $\sigma_1, \sigma_2, \ldots, \sigma_{2m}$ of $\pm 1$-valued labels. 

% Our refutation algorithm runs the agnostic learning algorithm on example-label pair $(x_i,\sigma_i)$ for $1 \leq i \leq m$ with error parameter $\epsilon_0/4.$ Let $h$ be the function output by the algorithm. Let $\cor_h = \frac{1}{m}\sum_{i =m+1}^{2m} \sigma_i \cdot h(x_i).$ If $\cor_h \geq \epsilon_0/2$ then output $\unclear$ otherwise output $\noise.$

% Let us analyze this procedure now. Suppose first that there exists a $c \in \C$ such that $\frac{1}{m}\sum_{ i =1}^m c(x_i) \sigma_i > \epsilon_0$. Then, by the definition of agnostic learning and standard union bound, with probability at least $2/3$ both over the randomness of the learner and the input sample, the output hypothesis $h$ satisfies: $\one{h(x)\ne y} < \frac{\epsilon_0}{2}$ Thus, in this case, the refutation algorithm outputs $\noise$  with probability at most $1/3$,  as desired.

% Next suppose $\sigma_i$s are i.i.d. uniform Rademacher variables. Then, since $\sigma_{m+1},\ldots, \sigma_{2m}$ are independent of $\sigma_1,\ldots, \sigma_m$, $\cor_h \leq \frac{4}{\sqrt{m}} < \epsilon_0/2$ with probability at least $2/3$. Thus, in this case, we output $\noise$ with probability at least $2/3$ as required.
\end{proof}

We now prove the other direction:

% \begin{lemma}[From Refutation to Learning]
% Let $\C$ be a concept class satisfying $\cR_{T(n),\delta}(\C) =  m(n,\delta) = m .$ Then, there's an $\epsilon$-agnostic learning algorithm for $\C$ over $\cD$ running in time $  .$ %distribution $\cD$ with error $\epsilon$ that runs in time $.$
% % Suppose that the refutation complexity of a class of Boolean concepts $\C$ with respect to a distribution $\cD$ at a running time of $T(n)$ is $m = \cR_{T(n)}(\C).$ Then, there's an agnostic learner for $\C$ with respect to $\cD$ with error parameter $\epsilon_0/2$ that runs in time $\poly(n) \poly(m) T(n).$
% \end{lemma}

\begin{lemma}[Learning by Refutation] \label{lem:refutation-to-learning}
Suppose that the $\delta$-refutation complexity of a class of Boolean concepts $\C$ with respect to a distribution $\cD$ at a running time $T(n)$ is $m = \cR_{T(n),\delta}(\C).$ Then, there's an algorithm that runs in time $T(n) \frac{m^2}{\epsilon^2}$ and uses $ O(\frac{m^3}{\epsilon^2})$ samples to $(\delta+\epsilon)$-agnostically learn $\C$ on $\cD$.
\end{lemma}


The proof is in two steps. In the first step, we show that the refutation algorithm yields a weak agnostic learner for $\C$ with respect to the distribution $\cD$. In the second step, we use the distribution specific agnostic boosting algorithm (see \cite{DBLP:conf/nips/KalaiK09}) to boost the accuracy of the weak learner to obtain an agnostic learner. We start by defining a weak-agnostic learner :

\begin{definition}[Weak Agnostic Learner]
An $(\gamma,\alpha)$-weak agnostic learner for a Boolean concept class $\C$ over a distribution $\cD$ is an algorithm that takes input random examples from a distribution $\cD'$ on example-label pairs $(x,y)$ such that the marginal on $x$ is $\cD$ such that with probability at least $3/4$ over its random input outputs a (randomized) hypothesis $h:\on^n \rightarrow \on$ such that $\E_{(x,y) \sim \cD'}[ y \cdot h(x) ]\geq \gamma (\sup_{c \in \C} \E_{(x,y) \sim \cD'}[y \cdot c(x)]) - \alpha.$
\end{definition}


\begin{lemma}[Refutation to Weak Agnostic Learner]
\label{lem:reftolearn}
Suppose that the $\delta$-refutation complexity of a class of Boolean concepts $\C$ with respect to a distribution $\cD$ at a running time $T(n)$ is $m = \cR_{T(n),\delta}(\C).$ Then, there's an $(\gamma,\alpha)$-weak agnostic learner for $\C$ on distribution $\cD$ that runs in time $T(n)$ and samples $m(n)$ where $\alpha = \delta \cdot \gamma$, $\gamma = \frac{2}{3m}.$
\end{lemma}


We describe a natural class of candidates for a weak learner that come out of running the refutation algorithm on appropriately chosen hybrids of the distribution $\cD'$ and $\cD \times \U_1.$ We begin by defining a class of $2(m+2)$ different functions denoted by $W_{i,b}:\on^n \rightarrow \zo$ for $0 \leq i \leq m+1$ and $b \in \pm 1$ produced by taking these hybrids. Our weak learners will be a simple transformation of this class.

\newcommand{\algnametwo}{3.1 \xspace}
\begin{center}
\fbox{\begin{minipage}{6in} 
\begin{center}
\textbf{\algnametwo Hybrid Functions $W_{i,b}$ } 
\end{center}

\begin{description}
\item[Input:] $x \in \R^n$, $b \in \on$.
\item[Output:] $W_{i,b}(x) = z \in \on.$ 
\item[Operation:] ~
\begin{enumerate}
\item Draw $(x_{1}, \sigma_{1}), \ldots, (x_{i-1},\sigma_{i-1})$ i.i.d. from $\cD \times \U_1$.  Draw $(x_{i+1}, y_{i+1}), (x_{i+2}, y_{i+2}) \ldots, (x_{m}, y_{m})$ i.i.d. from $\cD'$. 
\item Run the $\delta$-refutation algorithm on input\\ $(x_1,\sigma_1), (x_2, \sigma_2), \ldots, (x_{i-1},\sigma_{i-1}), (x,b), (x_{i+1},y_{i+1}), \ldots, (x_{m}, y_m)$.
\item Let $W_{i,b} = 1$ if the refutation algorithm returns $\unclear$ and $0$ otherwise.
\end{enumerate}
\end{description}
\end{minipage}}
\end{center}


We make some simple observations about $W_{i,b}$ that will come handy in the argument below.

Observe that $W_{m+1,b}$ is the function that evaluates to 1 if the output of the refutation algorithm on examples drawn from $\cD$ and labels i.i.d Rademacher variables is $\unclear$. On the other hand, $W_{0,b}$ is the function obtained when the refutation algorithm is run on example-label pairs from $\cD$. Finally, observe that 
\begin{equation}
\label{eq:randomizing-planting} \E_{b \sim \U_1} \E[ W_{i,b}(x)] = \E_{ (x,y) \sim \cD} \E[W_{i+1,y}(x)]
\end{equation}
Here, the inside expectation is over all the random choices within the procedure for computing $W_{i,b}$s above. We can now present our candidate weak learners.


\paragraph{Candidate Weak Learners} For every $0 \leq i \leq m+1$, let $h_i(x) = W_{i,+1}(x) - W_{i,-1}(x).$


\begin{proof}[Proof of Lemma \ref{lem:reftolearn}]
Our weak learning algorithm is given access to random labeled examples from a distribution $\cD'$ on $\R^n \otimes \{ \pm 1\}.$ The weak learner will draw a sample from $\cD'$ of size $O(\log{m})$ from $\cD'$ and chooses the $h_i$ that has the maximum correlation with the labels. Observe that with $O(\log{(m)})$ samples, the correlations of $h_i$ on $\cD'$ will be faithfully preserved with $2/3$ probability. Thus, to complete the proof, we only need to argue that one of the $h_i$s is always an $(\alpha,\gamma)$-weak learner.

 To show this, we must argue that there exists an $0\leq i \leq m+1$ such that:

\[
\E_{(x,y) \sim \cD'}[ y \cdot h_i(x) ] \geq \frac{2}{3m} \sup_{c \in \C} \E_{(x,y) \sim \cD'}[ c(x) \cdot y] - \frac{2}{3m} \delta.
\]

Observe that the guarantees of the weak learner are trivial if $\sup_{c \in \C} \E_{(x,y) \sim \cD'}[ y \cdot c(x)] < \delta.$ Thus assume that $\sup_{c \in \C} \E_{(x,y) \sim \cD'}[ y \cdot c(x)] > \delta.$ In this case, we will show that $\E_{(x,y) \sim \cD'}[h_i(x) y] \geq \frac{2}{3m}\geq \frac{2}{3m} \sup_{c \in \C} \E_{(x,y) \sim \cD'}[ c(x) \cdot y] - \frac{2}{3m}\delta.$


Now, observe that over the randomness of both the refutation algorithm and over the draw of i.i.d. sample from $\cD'$ of size $m = S(n)$, $\E[ W_{0,b} (x)] \geq 2/3$ and $\E[W_{m+1,b}(x)] \leq 1/3$ for any $b$. Thus, $$\sum_{i = 0}^m \E[ W_{i,y}(x) - W_{i+1,y}(x)] \geq 1/3,$$ where the expectation is over the randomness in the draw $(x,y) \sim \cD'$ and over the randomness in $W_{i,y}$ for $0 \leq i \leq m+1.$

Thus, there must exist an $i$ such that $\E[ W_{i,y}(x) - W_{i+1,y}(x)] > 1/3m.$ Observe that by construction 
\begin{multline} W_{i,y}(x) = \frac{y+1}{2} \cdot W_{i,1}(x) - \frac{y-1}{2} W_{i,-1}(x) = y \cdot \frac{W_{i,1}(x) - W_{i,-1}(x)}{2} + \frac{1}{2} (W_{i,1}(x) + W_{i,-1}(x)) \\= \frac{1}{2} y \cdot h_i(x)  + \frac{1}{2} (W_{i,1}(x) + W_{i,-1}(x)). \label{eq:whatever}\end{multline}

Next, observe that by \eqref{eq:randomizing-planting}, $\E[\frac{1}{2} (W_{i,1}(x) + W_{i,-1}(x))] = \E[ W_{i+1,y}(x)].$ 
Taking expectations on both sides of \eqref{eq:whatever} and rearranging, we have: $\E[ y \cdot h_i(x)] \geq \frac{2}{3m}.$ 

This establishes that for $\gamma = \frac{2}{3m}$ and $\alpha = \delta \cdot \gamma$ our algorithm returns $(\alpha, \gamma)$-weak agnostic learner as desired.
\end{proof}

We can now use boosting to get a strong agnostic learner for $\C$ over $\cD$ by using the weak learning algorithm along with a boosting algorithm. Specifically, we will use the result of Kalai and Kanade \cite{DBLP:conf/nips/KalaiK09}  (see also \cite{feldman2010distribution}) who showed the following agnostic boosting algorithm that takes a $( \gamma, \alpha )$-weak learner and outputs a hypothesis whose error is competitive within $\alpha$ with respect to the best fitting hypothesis from the class $\C$. 

\begin{fact}[Agnostic Boosting \cite{DBLP:conf/nips/KalaiK09}] \label{fact:boosting}
Let $\C$ be a class of Boolean concepts.
Let $\cD$ be a distribution on $\on^n$ and $\epsilon > 0.$

There's an algorithm that takes random labeled examples from a distribution $\cD'$ on example-label pairs $(x,y)$ such that the marginal on $x$ is $\cD$, invokes a $(\gamma,\alpha)$-weak learner for $\C$ $O(\frac{1}{\gamma^2 \epsilon^2})$ times and outputs a hypothesis $h: \on^n \rightarrow \on$ such that $$\E_{(x,y) \sim \cD'}\left[ \one{h(x)\ne y} \right] \leq \inf_{c \in \C} \E_{(x,y) \sim \cD'}\left[\one{c(x)\ne y}\right] + \alpha/\gamma + \epsilon.$$
The algorithm needs $S(n) \cdot O(\frac{1}{\gamma^2 \epsilon^2})$ samples and runs in time $T(n) \cdot O(\frac{1}{\gamma^2 \epsilon^2})$ where $S(n)$ and $T(n)$ are the sample complexity and the running time respectively of the $(\gamma, \alpha)$-weak agnostic learner.
\end{fact}{}

We get Lemma \ref{lem:refutation-to-learning} as an immediate corollary of Fact \ref{fact:boosting} and Lemma \ref{lem:reftolearn}.




% \section{A Sample Complexity Lower Bound for Agnostically Learning Disjunctions}

% Our lower bound is based on an strong extension of Feige's hypothesis \cite{DBLP:conf/coco/Feige02} for strongly refuting $k$-XOR CSP. Similar hypothesis (for $k$-SAT instead of $k$-XOR) were used by Daniely \cite{DBLP:conf/stoc/Daniely16,daniely2016complexity} to show hardness of PAC-learning DNFs and halfspaces over arbitrary distributions.  

% We first define the problem of refuting $k$-XOR.

% \begin{definition}[Refuting $k$-XOR]
% In the refutation problem for a $k$-XOR, we are given $m$ $k$-tuples $(i_1, i_2, \ldots, i_k)$ for $1 \leq i \leq m$ chosen uniformly from the set of all $k$-tuples ${[n] \choose k}$ over $n$ Boolean variables (i.e over $\on$) and $m$ bits $\sigma_1, \sigma_2, \ldots, \sigma_m \sim \{ \pm 1\}.$ For any $x$, let $\val(x)$ be the number of $k$-tuples $(i_1, i_2, \ldots, i_k)$ in the input such that $\Pi_{j = 1}^k x_{i_j} = \sigma_i.$ 

% The goal is to output $\noise$ or $\unclear$ with the following guarantees:
% \begin{enumerate}
% \item If the output is $\noise$, then $\frac{1}{m} \sup_{x \in \on^n} \val(x) \leq \delta.$ 
% \item If $\sigma_i$ are chosen i.i.d. according to $\U_1$, then, $\Pr[ \text{ output = } \noise] \geq 2/3.$
% 	\end{enumerate}
% \end{definition}
 
% \begin{hypothesis}[Hardness of Strong Refutation of $k$-XOR]
% Any algorithm 
% \end{hypothesis}
% \begin{theorem}
% There exists a distribution $\cD$ on $\on^n$ such that any $\delta$-agnostic learner for the class of disjunctions on $\cD$ requires $n^{\Omega(\log{(1/\delta)})}$ samples. 
% \end{theorem}







% Lemma \FIXME immediately reduces this task to showing the following lemma.



% \begin{lemma}
% There exists a distribution $\cD$ such that the $\delta$-refutation complexity of the class of disjunctions on $\cD$ is at least $n^{\Omega(\log{(1/\delta)})}.$
% \end{lemma}

% \begin{proof}


% \end{proof}



==> preamble/macros-custom.tex <==
% algorithm packages


%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{algpseudocode}

%\algnewcommand\algorithmicinput{\textbf{Input:}}
%\algnewcommand\INPUT{\item[\algorithmicinput]}
%\algnewcommand\algorithmicoutput{\textbf{Output:}}
%\algnewcommand\OUTPUT{\item[\algorithmicoutput]}

% paper-specific packages
\usepackage{relsize}
\usepackage[font=footnotesize]{caption}
\usepackage{appendix,color}


% abbreviations and paper-specific macros

% math
\newcommand{\D}{\mathcal{D}}
\newcommand{\sphere}{\bbS^{n-1}}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\lamax}{\lambda_{\mathrm{max}}}
\newcommand{\Sn}{\mathbb{S}^{n-1}}
\DeclareMathOperator{\Id}{\mathrm{Id}}
\DeclareMathOperator{\F}{\mathbb{F}}
\DeclareMathOperator{\codim}{codim}

% not math
\DeclareUrlCommand\email{}
\newcommand{\whp}{\text{w.h.p.}}
\newcommand{\wovp}{\text{w.ov.p.}\xspace}
\newcommand{\YES}{\textsc{yes}\xspace}
\newcommand{\NO}{\textsc{no}\xspace}

\newcommand{\wovple}{\hspace{-3mm}\stackrel{\text{\wovp}}{\le}}
\newcommand{\wovpeq}{\hspace{-3mm}\stackrel{\text{\wovp}}{=}}
\newcommand{\wovpge}{\hspace{-3mm}\stackrel{\text{\wovp}}{\ge}}
\newcommand{\aasle}{\hspace{-1.5mm}\stackrel{\text{a.a.s.}}\le}

\newcommand{\Pisymm}{\Pi_{\mathrm{symm}}}
\newcommand{\Pisym}{\Pi_{\mathrm{sym}}}

%added by TM
\newcommand{\inner}[1]{\langle #1 \rangle}
\newcommand{\sosle}{\preceq}
\newcommand{\sosge}{\succeq}

\DeclareMathOperator{\tE}{\tilde{\mathbb E}}
\DeclareMathOperator{\tO}{\tilde{O}}
\DeclareMathOperator{\zo}{\{0,1\}}


\DeclareMathOperator*{\pE}{\tilde{\mathbb E}}

\newcommand{\bT}{\mathbf{T}}
\newcommand{\ot}{\otimes}
\newcommand{\tr}{\textup{tr}}
\newcommand{\diag}{\textup{diag}}

\let\pref=\prettyref

% transpose
% http://tex.stackexchange.com/questions/204892/visually-appealing-subscripts-with-intercal
% http://tex.stackexchange.com/questions/30619/what-is-the-best-symbol-for-vector-matrix-transpose
\newcommand*{\transpose}[1]{{#1}{}^{\mkern-4mu\intercal}}
\newcommand*{\vardyad}[1]{#1^{\vphantom{\intercal}}#1^{\intercal}}
\newcommand*{\dyad}[1]{#1#1{}^{\mkern-4mu\intercal}}

% \let\Id\undefined
% \newcommand*{\Id}{I}

% span of subspace -- temporary

\newcommand{\sspan}{\textup{span}}
\newcommand{\1}{\bm{1}}

\newcommand{\rl}[1]{\color{red}{R:#1}\color{black}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../planted"
%%% End:


==> preamble/macros.tex <==
% {{{ etex }}}

\usepackage{etex}

% {{{ nag }}}

\usepackage[l2tabu, orthodox]{nag}

% {{{ common }}}

\usepackage{xspace,enumerate}

\usepackage[dvipsnames]{xcolor}

\usepackage[T1]{fontenc}
\usepackage[full]{textcomp}

% {{{ babelamerican }}}
\usepackage[american]{babel}

% {{{ mathtools }}}

\usepackage{mathtools}


% {{{ boldmath }}}

% fix for "too many math alphabets" problem
\newcommand\hmmax{0} % default 3
% \usepackage{bm}

% \usepackage{stmaryrd}


% {{{ amsthm }}}
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}

\newtheorem{subclaim}{Claim}[theorem]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem*{fact*}{Fact}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem*{hypothesis*}{Hypothesis}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{protocol}[theorem]{Protocol}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem*{claim*}{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}



% {{{ geometry-nice }}}


\ifnum\writemode=1
\usepackage[
letterpaper,
top=1.2in,
bottom=1.2in,
left=1in,
right=1in]{geometry}

\pagestyle{empty}
\fi

\ifnum\writemode=0
\usepackage[
letterpaper,
top=0.7in,
bottom=0.9in,
left=1in,
right=1in]{geometry}
\fi

% {{{ fonts }}}

\usepackage{newpxtext} % T1, lining figures in math, osf in text
\usepackage{textcomp} % required for special glyphs
\usepackage[varg,bigdelims]{newpxmath}
\usepackage[scr=rsfso]{mathalfa}% \mathscr is fancier than \mathcal
\usepackage{bm} % load after all math to give access to bold math
% \useosf %no longer needed
\linespread{1.1}% Give Palatino more leading (space between lines)
\let\mathbb\varmathbb

% {{{ showkeys }}}

\ifnum\showkeys=1
\usepackage[color]{showkeys}
\fi

% {{{ hyperref-option2 }}}

\ifnum\showcolorlinks=1
\usepackage[
pagebackref,
% letterpaper=true,
colorlinks=true,
urlcolor=blue,
linkcolor=blue,
citecolor=OliveGreen,
]{hyperref}
\fi

\ifnum\showcolorlinks=0
\usepackage[
pagebackref,
% letterpaper=true,
colorlinks=false,
pdfborder={0 0 0}
]{hyperref}
\fi


\usepackage[capitalise,nameinlink]{cleveref}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{definition}{Definition}{Definitions}

% {{{ prettyref }}}

% \usepackage{prettyref}

% % From manual:
% % \newrefformat{eq}{\textup{(\ref{#1})}}
% % \newrefformat{lem}{Lemma~\ref{#1}}
% % \newrefformat{thm}{Theorem~\ref{#1}}
% % \newrefformat{cha}{Chapter~\ref{#1}}
% % \newrefformat{sec}{Section~\ref{#1}}
% % \newrefformat{tab}{Table~\ref{#1} on page~\pageref{#1}}
% % \newrefformat{fig}{Figure~\ref{#1} on page~\pageref{#1}}

% \newcommand{\savehyperref}[2]{\texorpdfstring{\hyperref[#1]{#2}}{#2}}

% \newrefformat{eq}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
% \newrefformat{eqn}{\savehyperref{#1}{\textup{(\ref*{#1})}}}
% \newrefformat{lem}{\savehyperref{#1}{Lemma~\ref*{#1}}}
% \newrefformat{def}{\savehyperref{#1}{Definition~\ref*{#1}}}
% \newrefformat{thm}{\savehyperref{#1}{Theorem~\ref*{#1}}}
% \newrefformat{cor}{\savehyperref{#1}{Corollary~\ref*{#1}}}
% \newrefformat{cha}{\savehyperref{#1}{Chapter~\ref*{#1}}}
% \newrefformat{sec}{\savehyperref{#1}{Section~\ref*{#1}}}
% \newrefformat{app}{\savehyperref{#1}{Appendix~\ref*{#1}}}
% \newrefformat{tab}{\savehyperref{#1}{Table~\ref*{#1}}}
% \newrefformat{fig}{\savehyperref{#1}{Figure~\ref*{#1}}}
% \newrefformat{hyp}{\savehyperref{#1}{Hypothesis~\ref*{#1}}}
% \newrefformat{alg}{\savehyperref{#1}{Algorithm~\ref*{#1}}}
% \newrefformat{rem}{\savehyperref{#1}{Remark~\ref*{#1}}}
% \newrefformat{item}{\savehyperref{#1}{Item~\ref*{#1}}}
% \newrefformat{step}{\savehyperref{#1}{step~\ref*{#1}}}
% \newrefformat{conj}{\savehyperref{#1}{Conjecture~\ref*{#1}}}
% \newrefformat{fact}{\savehyperref{#1}{Fact~\ref*{#1}}}
% \newrefformat{prop}{\savehyperref{#1}{Proposition~\ref*{#1}}}
% \newrefformat{prob}{\savehyperref{#1}{Problem~\ref*{#1}}}
% \newrefformat{claim}{\savehyperref{#1}{Claim~\ref*{#1}}}
% \newrefformat{relax}{\savehyperref{#1}{Relaxation~\ref*{#1}}}
% \newrefformat{red}{\savehyperref{#1}{Reduction~\ref*{#1}}}
% \newrefformat{part}{\savehyperref{#1}{Part~\ref*{#1}}}



% {{{ sref }}}

% short section reference
\newcommand{\Sref}[1]{\hyperref[#1]{\S\ref*{#1}}}

% {{{ nicefrac }}}
% commands for fractions
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}

\let\nfrac=\nicefrac
\let\ffrac=\flatfrac
% similar commands: tfrac,dfrac

\newcommand{\half}{\nicefrac12}
\newcommand{\onequarter}{\nicefrac14}
\newcommand{\threequarter}{\nicefrac34}

% {{{ microtype-option }}}

\ifnum\usemicrotype=1
\usepackage{microtype}
\fi

% {{{ authornotes }}}
\ifnum\showauthornotes=1
\newcommand{\Authornote}[2]{{\sffamily\small\color{red}{[#1: #2]}}}
\newcommand{\Authornotecolored}[3]{{\sffamily\small\color{#1}{[#2: #3]}}}
\newcommand{\Authorcomment}[2]{{\sffamily\small\color{gray}{[#1: #2]}}}
\newcommand{\Authorstartcomment}[1]{\sffamily\small\color{gray}[#1: }
\newcommand{\Authorendcomment}{]\rmfamily\normalsize\color{black}}
\newcommand{\Authorfnote}[2]{\footnote{\color{red}{#1: #2}}}
\newcommand{\Authorfixme}[1]{\Authornote{#1}{\textbf{??}}}
\newcommand{\Authormarginmark}[1]{\marginpar{\textcolor{red}{\fbox{\Large #1:!}}}}
\else
\newcommand{\Authornote}[2]{}
\newcommand{\Authornotecolored}[3]{}
\newcommand{\Authorcomment}[2]{}
\newcommand{\Authorstartcomment}[1]{}
\newcommand{\Authorendcomment}{}
\newcommand{\Authorfnote}[2]{}
\newcommand{\Authorfixme}[1]{}
\newcommand{\Authormarginmark}[1]{}
\fi

\newcommand{\Dnote}{\Authornote{D}}
%\newcommand{\Tnote}{\Authornotecolored{blue}{T}}
\newcommand{\TMnote}{\Authornotecolored{blue}{T}}
\newcommand{\Inote}{\Authornotecolored{ForestGreen}{I}}
\newcommand{\inote}{\Inote}
\newcommand{\Gnote}{\Authornote{G}}
\newcommand{\Jcomment}{\Authorcomment{J}}
\newcommand{\Dcomment}{\Authorcomment{D}}
\newcommand{\Dstartcomment}{\Authorstartcomment{D}}
\newcommand{\Dendcomment}{\Authorendcomment}
\newcommand{\Dfixme}{\Authorfixme{D}}
\newcommand{\Dmarginmark}{\Authormarginmark{D}}
\newcommand{\Dfnote}{\Authorfnote{D}}
\newcommand{\one}[1]{\mathbf{1}\left[#1\right]}
\newcommand{\Pnote}{\Authornote{P}}
\newcommand{\Pfnote}{\Authorfnote{P}}

\newcommand{\PRnote}{\Authornote{PR}}
\newcommand{\PRfnote}{\Authorfnote{PR}}

\newcommand{\PTnote}{\Authornote{PT}}
\newcommand{\PTfnote}{\Authorfnote{PT}}

\newcommand{\PGnote}{\Authornote{PG}}
\newcommand{\PGfnote}{\Authorfnote{PG}}

\newcommand{\Bnote}{\Authornote{B}}
\newcommand{\Bfnote}{\Authorfnote{B}}

\definecolor{forestgreen(traditional)}{rgb}{0.0, 0.27, 0.13}
\newcommand{\Jnote}{\Authornotecolored{forestgreen(traditional)}{J}}
\newcommand{\Jfnote}{\Authorfnote{J}}


\newcommand{\Mnote}{\Authornote{M}}
\newcommand{\Mfnote}{\Authorfnote{M}}

\newcommand{\Rnote}{\Authornote{M}}
\newcommand{\Rfnote}{\Authorfnote{M}}

\newcommand{\Nnote}{\Authornote{N}}
\newcommand{\Nfnote}{\Authorfnote{N}}

\newcommand{\Snote}{\Authornote{S}}
\newcommand{\Sfnote}{\Authorfnote{S}}


% {{{ fixme }}}

% place red exclamation mark in margin
%\newcommand{\redmarginmarker}{\marginpar{\textcolor{red}{\fbox{\Large !}}}}
\newcommand{\redmarginmarker}{}

% short indicator for places that need fixing
\newcommand{\FIXME}{\textbf{\textcolor{red}{??}}\redmarginmarker}

\ifnum\showfixme=0
\renewcommand{\FIXME}{}
\fi


% {{{ boxedminipage }}}
\usepackage{boxedminipage}

\newenvironment{mybox}
{\center \noindent\begin{boxedminipage}{1.0\linewidth}}
{\end{boxedminipage}
\noindent
}


% {{{ parentheses }}}
% various bracket-like commands
% round parentheses
\newcommand{\paren}[1]{(#1)}
\newcommand{\Paren}[1]{\left(#1\right)}
\newcommand{\bigparen}[1]{\big(#1\big)}
\newcommand{\Bigparen}[1]{\Big(#1\Big)}
% square brackets
\newcommand{\brac}[1]{[#1]}
\newcommand{\Brac}[1]{\left[#1\right]}
\newcommand{\bigbrac}[1]{\big[#1\big]}
\newcommand{\Bigbrac}[1]{\Big[#1\Big]}
\newcommand{\Biggbrac}[1]{\Bigg[#1\Bigg]}
% absolute value
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigabs}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigabs}[1]{\Big\lvert#1\Big\rvert}
% cardinality
\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Card}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigcard}[1]{\big\lvert#1\big\rvert}
\newcommand{\Bigcard}[1]{\Big\lvert#1\Big\rvert}
% set
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigset}[1]{\big\{#1\big\}}
\newcommand{\Bigset}[1]{\Big\{#1\Big\}}
% norm
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bignorm}[1]{\big\lVert#1\big\rVert}
\newcommand{\Bignorm}[1]{\Big\lVert#1\Big\rVert}
\newcommand{\Biggnorm}[1]{\Bigg\lVert#1\Bigg\rVert}
% 2-norm
\newcommand{\normt}[1]{\norm{#1}_2}
\newcommand{\Normt}[1]{\Norm{#1}_2}
\newcommand{\bignormt}[1]{\bignorm{#1}_2}
\newcommand{\Bignormt}[1]{\Bignorm{#1}_2}
% 2-norm squared
\newcommand{\snormt}[1]{\norm{#1}^2_2}
\newcommand{\Snormt}[1]{\Norm{#1}^2_2}
\newcommand{\bigsnormt}[1]{\bignorm{#1}^2_2}
\newcommand{\Bigsnormt}[1]{\Bignorm{#1}^2_2}
% norm squared
\newcommand{\snorm}[1]{\norm{#1}^2}
\newcommand{\Snorm}[1]{\Norm{#1}^2}
\newcommand{\bigsnorm}[1]{\bignorm{#1}^2}
\newcommand{\Bigsnorm}[1]{\Bignorm{#1}^2}
% 1-norm
\newcommand{\normo}[1]{\norm{#1}_1}
\newcommand{\Normo}[1]{\Norm{#1}_1}
\newcommand{\bignormo}[1]{\bignorm{#1}_1}
\newcommand{\Bignormo}[1]{\Bignorm{#1}_1}
% infty-norm
\newcommand{\normi}[1]{\norm{#1}_\infty}
\newcommand{\Normi}[1]{\Norm{#1}_\infty}
\newcommand{\bignormi}[1]{\bignorm{#1}_\infty}
\newcommand{\Bignormi}[1]{\Bignorm{#1}_\infty}
% inner product
\newcommand{\iprod}[1]{\langle#1\rangle}
\newcommand{\Iprod}[1]{\left\langle#1\right\rangle}
\newcommand{\bigiprod}[1]{\big\langle#1\big\rangle}
\newcommand{\Bigiprod}[1]{\Big\langle#1\Big\rangle}


% {{{ probability }}}
% expectation, probability, variance
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathbb{V}}

\DeclareMathOperator*{\E}{\Esymb}
\DeclareMathOperator*{\Var}{\Vsymb}
\DeclareMathOperator*{\ProbOp}{\Psymb}

\renewcommand{\Pr}{\ProbOp}

% TODO: make case distinction if optional argument is not set
\newcommand{\prob}[1]{\Pr\set{#1}}
\newcommand{\Prob}[2][]{\Pr_{{#1}}\Set{#2}}

\newcommand{\ex}[1]{\E\brac{#1}}
\newcommand{\Ex}[2][]{\E_{{#1}}\Brac{#2}}
\newcommand{\varex}[1]{\E\paren{#1}}
\newcommand{\varEx}[1]{\E\Paren{#1}}

%\newcommand{\given}{\;\middle\vert\;}
\newcommand{\given}{\mathrel{}\middle\vert\mathrel{}}
%\newcommand{\given}{\mathrel{}\middle|\mathrel{}}

% {{{ mathfonts }}}

% \usepackage{dsfont}
% \usepackage{yfonts}
% \usepackage{mathrsfs}


% {{{ miscmacros }}}

% middle delimiter in the definition of a set
\newcommand{\suchthat}{\;\middle\vert\;}

% tensor product
\newcommand{\tensor}{\otimes}

% add explanations to math displays
\newcommand{\where}{\text{where}}
\newcommand{\textparen}[1]{\text{(#1)}}
\newcommand{\using}[1]{\textparen{using #1}}
\newcommand{\smallusing}[1]{\text{(\small using #1)}}
\ifx\because\undefined
\newcommand{\because}[1]{\textparen{because #1}}
\else
\renewcommand{\because}[1]{\textparen{because #1}}
\fi
\newcommand{\by}[1]{\textparen{by #1}}


% spectral order (Loewner order)
\newcommand{\sge}{\succeq}
\newcommand{\sle}{\preceq}

% smallest and largest eigenvalue
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\lmax}{\lambda_{\max}}

\newcommand{\signs}{\set{1,-1}}
\newcommand{\varsigns}{\set{\pm 1}}
\newcommand{\maximize}{\mathop{\textrm{maximize}}}
\newcommand{\minimize}{\mathop{\textrm{minimize}}}
\newcommand{\subjectto}{\mathop{\textrm{subject to}}}

\renewcommand{\ij}{{ij}}

% symmetric difference
\newcommand{\symdiff}{\Delta}
\newcommand{\varsymdiff}{\bigtriangleup}

% set of bits
\newcommand{\bits}{\{0,1\}}
\newcommand{\sbits}{\{\pm1\}}

% no stupid bullets for itemize environmentx
% \renewcommand{\labelitemi}{--}

% control white space of list and display environments
\newcommand{\listoptions}{\labelsep0mm\topsep-0mm\itemindent-6mm\itemsep0mm}
\newcommand{\displayoptions}[1]{\abovedisplayshortskip#1mm\belowdisplayshortskip#1mm\abovedisplayskip#1mm\belowdisplayskip#1mm}

% short for emptyset
%\newcommand{\eset}{\emptyset}
% moved to mathabbreviations

% short for epsilon
%\newcommand{\e}{\epsilon}
% moved to mathabbreviations

% super index with parentheses
\newcommand{\super}[2]{#1^{\paren{#2}}}
\newcommand{\varsuper}[2]{#1^{\scriptscriptstyle\paren{#2}}}

% tensor power notation
\newcommand{\tensorpower}[2]{#1^{\tensor #2}}


% multiplicative inverse
\newcommand{\inv}[1]{{#1^{-1}}}

% dual element
\newcommand{\dual}[1]{{#1^*}}

% subset
%\newcommand{\sse}{\subseteq}
% moved to mathabbreviations

% vertical space in math formula
\newcommand{\vbig}{\vphantom{\bigoplus}}

% setminus
\newcommand{\sm}{\setminus}

% define something by an equation (display)
\newcommand{\defeq}{\stackrel{\mathrm{def}}=}


% define something by an equation (inline)
\newcommand{\seteq}{\mathrel{\mathop:}=}



% declare function f by $f \from X \to Y$
\newcommand{\from}{\colon}

% big middle separator (for conditioning probability spaces)
\newcommand{\bigmid}{~\big|~}
\newcommand{\Bigmid}{~\Big|~}
\newcommand{\Mid}{\;\middle\vert\;}

% better vector definition and some variations
%\renewcommand{\vec}[1]{{\bm{#1}}}
\newcommand{\bvec}[1]{\bar{\vec{#1}}}
\newcommand{\pvec}[1]{\vec{#1}'}
\newcommand{\tvec}[1]{{\tilde{\vec{#1}}}}

% punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

% inner product for matrices
\newcommand\bdot\bullet

% transpose
\newcommand{\trsp}[1]{{#1}^\dagger}

% indicator function / vector
\ifx\mathds\undefined % use double stroke fonts if available
\DeclareMathOperator{\Ind}{\mathbb{I}}
\else
\DeclareMathOperator{\Ind}{\mathds 1}}
\fi

% place a qed symbol inside display formula
%\qedhere

% {{{ superscripts }}}

\renewcommand{\th}{\textsuperscript{th}\xspace}
\newcommand{\st}{\textsuperscript{st}\xspace}
\newcommand{\nd}{\textsuperscript{nd}\xspace}
\newcommand{\rd}{\textsuperscript{rd}\xspace}


% {{{ mathoperators }}}
\DeclareMathOperator{\Inf}{Inf}
\DeclareMathOperator{\Tr}{Tr}
%\newcommand{\Tr}{\mathrm{Tr}}
\DeclareMathOperator{\SDP}{SDP}
\DeclareMathOperator{\sdp}{sdp}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\opt}{opt}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\qpoly}{qpoly}
\DeclareMathOperator{\qpolylog}{qpolylog}
\DeclareMathOperator{\qqpoly}{qqpoly}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Conv}{Conv}

\DeclareMathOperator{\rank}{rank}

% operators with limits
\DeclareMathOperator*{\median}{median}
\DeclareMathOperator*{\Median}{Median}

% smaller summation/product symbols
\DeclareMathOperator*{\varsum}{{\textstyle \sum}}
\DeclareMathOperator{\tsum}{{\textstyle \sum}}

\let\varprod\undefined

\DeclareMathOperator*{\varprod}{{\textstyle \prod}}
\DeclareMathOperator{\tprod}{{\textstyle \prod}}




% {{{ differentials }}}

\newcommand{\diffmacro}[1]{\,\mathrm{d}#1}

\newcommand{\dmu}{\diffmacro{\mu}}
\newcommand{\dgamma}{\diffmacro{\gamma}}
\newcommand{\dlambda}{\diffmacro{\lambda}}
\newcommand{\dx}{\diffmacro{x}}
\newcommand{\dt}{\diffmacro{t}}



% {{{ textabbreviations }}}

% some abbreviations
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\phd}{Ph.\,D.\xspace}
\newcommand{\msc}{M.\,S.\xspace}
\newcommand{\bsc}{B.\,S.\xspace}

\newcommand{\etal}{et al.\xspace}

\newcommand{\iid}{i.i.d.\xspace}

% {{{ foreignwords }}}

\newcommand\naive{na\"{\i}ve\xspace}
\newcommand\Naive{Na\"{\i}ve\xspace}
\newcommand\naively{na\"{\i}vely\xspace}
\newcommand\Naively{Na\"{\i}vely\xspace}




% {{{ names }}}
% Hungarian/Polish/East European names
\newcommand{\Erdos}{Erd\H{o}s\xspace}
\newcommand{\Renyi}{R\'enyi\xspace}
\newcommand{\Lovasz}{Lov\'asz\xspace}
\newcommand{\Juhasz}{Juh\'asz\xspace}
\newcommand{\Bollobas}{Bollob\'as\xspace}
\newcommand{\Furedi}{F\"uredi\xspace}
\newcommand{\Komlos}{Koml\'os\xspace}
\newcommand{\Luczak}{\L uczak\xspace}
\newcommand{\Kucera}{Ku\v{c}era\xspace}
\newcommand{\Szemeredi}{Szemer\'edi\xspace}
\newcommand{\Hastad}{H{\aa}stad\xspace}
\newcommand{\Hoelder}{H\"{o}lder\xspace}
\newcommand{\Holder}{\Hoelder}
\newcommand{\Brandao}{Brand\~ao\xspace}


% {{{ numbersets }}}
% number sets
\newcommand{\Z}{\mathbb Z}
\newcommand{\N}{\mathbb N}
\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\Rnn}{\R_+}
\newcommand{\varR}{\Re}
\newcommand{\varRnn}{\varR_+}
\newcommand{\varvarRnn}{\R_{\ge 0}}


% {{{ problems }}}

% macros to denote computational problems

% use texorpdfstring to avoid problems with hyperref (can use problem
% macros also in headings
\newcommand{\problemmacro}[1]{\texorpdfstring{\textup{\textsc{#1}}}{#1}\xspace}

\newcommand{\pnum}[1]{{\footnotesize #1}}

% list of problems
\newcommand{\uniquegames}{\problemmacro{unique games}}
\newcommand{\maxcut}{\problemmacro{max cut}}
\newcommand{\multicut}{\problemmacro{multi cut}}
\newcommand{\vertexcover}{\problemmacro{vertex cover}}
\newcommand{\balancedseparator}{\problemmacro{balanced separator}}
\newcommand{\maxtwosat}{\problemmacro{max \pnum{3}-sat}}
\newcommand{\maxthreesat}{\problemmacro{max \pnum{3}-sat}}
\newcommand{\maxthreelin}{\problemmacro{max \pnum{3}-lin}}
\newcommand{\threesat}{\problemmacro{\pnum{3}-sat}}
\newcommand{\labelcover}{\problemmacro{label cover}}
\newcommand{\setcover}{\problemmacro{set cover}}
\newcommand{\maxksat}{\problemmacro{max $k$-sat}}
\newcommand{\mas}{\problemmacro{maximum acyclic subgraph}}
\newcommand{\kwaycut}{\problemmacro{$k$-way cut}}
\newcommand{\sparsestcut}{\problemmacro{sparsest cut}}
\newcommand{\betweenness}{\problemmacro{betweenness}}
\newcommand{\uniformsparsestcut}{\problemmacro{uniform sparsest cut}}
\newcommand{\grothendieckproblem}{\problemmacro{Grothendieck problem}}
\newcommand{\maxfoursat}{\problemmacro{max \pnum{4}-sat}}
\newcommand{\maxkcsp}{\problemmacro{max $k$-csp}}
\newcommand{\maxdicut}{\problemmacro{max dicut}}
\newcommand{\maxcutgain}{\problemmacro{max cut gain}}
\newcommand{\smallsetexpansion}{\problemmacro{small-set expansion}}
\newcommand{\minbisection}{\problemmacro{min bisection}}
\newcommand{\minimumlineararrangement}{\problemmacro{minimum linear arrangement}}
\newcommand{\maxtwolin}{\problemmacro{max \pnum{2}-lin}}
\newcommand{\gammamaxlin}{\problemmacro{$\Gamma$-max \pnum{2}-lin}}
\newcommand{\basicsdp}{\problemmacro{basic sdp}}
\newcommand{\dgames}{\problemmacro{$d$-to-1 games}}
\newcommand{\maxclique}{\problemmacro{max clique}}
\newcommand{\densestksubgraph}{\problemmacro{densest $k$-subgraph}}


% {{{ alphabet }}}

\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\cH}{\mathcal H}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

\newcommand{\scrA}{\mathscr A}
\newcommand{\scrB}{\mathscr B}
\newcommand{\scrC}{\mathscr C}
\newcommand{\scrD}{\mathscr D}
\newcommand{\scrE}{\mathscr E}
\newcommand{\scrF}{\mathscr F}
\newcommand{\scrG}{\mathscr G}
\newcommand{\scrH}{\mathscr H}
\newcommand{\scrI}{\mathscr I}
\newcommand{\scrJ}{\mathscr J}
\newcommand{\scrK}{\mathscr K}
\newcommand{\scrL}{\mathscr L}
\newcommand{\scrM}{\mathscr M}
\newcommand{\scrN}{\mathscr N}
\newcommand{\scrO}{\mathscr O}
\newcommand{\scrP}{\mathscr P}
\newcommand{\scrQ}{\mathscr Q}
\newcommand{\scrR}{\mathscr R}
\newcommand{\scrS}{\mathscr S}
\newcommand{\scrT}{\mathscr T}
\newcommand{\scrU}{\mathscr U}
\newcommand{\scrV}{\mathscr V}
\newcommand{\scrW}{\mathscr W}
\newcommand{\scrX}{\mathscr X}
\newcommand{\scrY}{\mathscr Y}
\newcommand{\scrZ}{\mathscr Z}

\newcommand{\bbB}{\mathbb B}
\newcommand{\bbS}{\mathbb S}
\newcommand{\bbR}{\mathbb R}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbI}{\mathbb I}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbP}{\mathbb P}
\newcommand{\bbE}{\mathbb E}
\newcommand{\bbN}{\mathbb N}

\newcommand{\sfE}{\mathsf E}


% {{{ leqslant }}}
% slanted lower/greater equal signs
\renewcommand{\leq}{\leqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\ge}{\geqslant}


% {{{ draftbox }}}
\ifnum\showdraftbox=1
\newcommand{\draftbox}{\begin{center}
  \fbox{%
    \begin{minipage}{2in}%
      \begin{center}%
%        \begin{Large}%
          \Large\textsc{Working Draft}\\%
%        \end{Large}\\
        Please do not distribute%
      \end{center}%
    \end{minipage}%
  }%
\end{center}
\vspace{0.2cm}}
\else
\newcommand{\draftbox}{}
\fi


% {{{ varepsilon }}}

\let\epsilon=\varepsilon

% {{{ numberequationwithinsection }}}
\numberwithin{equation}{section}


% {{{ restate }}}
% set of macros to deal with restating theorem environments (or anything
% else with a label)

% stolen from Boaz's latex macros

\newcommand\MYcurrentlabel{xxx}

% \MYstore{A}{B} assigns variable A value B
\newcommand{\MYstore}[2]{%
  \global\expandafter \def \csname MYMEMORY #1 \endcsname{#2}%
}

% \MYload{A} outputs value stored for variable A
\newcommand{\MYload}[1]{%
  \csname MYMEMORY #1 \endcsname%
}

% new label command, stores current label in \MYcurrentlabel
\newcommand{\MYnewlabel}[1]{%
  \renewcommand\MYcurrentlabel{#1}%
  \MYoldlabel{#1}%
}

% new label command that doesn't do anything
\newcommand{\MYdummylabel}[1]{}

\newcommand{\torestate}[1]{%
  % overwrite label command
  \let\MYoldlabel\label%
  \let\label\MYnewlabel%
  #1%
  \MYstore{\MYcurrentlabel}{#1}%
  % restore old label command
  \let\label\MYoldlabel%
}

\newcommand{\restatetheorem}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{theorem*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{theorem*}
  \let\label\MYoldlabel
}

\newcommand{\restatelemma}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{lemma*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{lemma*}
  \let\label\MYoldlabel
}

\newcommand{\restateprop}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{proposition*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{proposition*}
  \let\label\MYoldlabel
}

\newcommand{\restatefact}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{fact*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{fact*}
  \let\label\MYoldlabel
}

\newcommand{\restate}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \MYload{#1}
  \let\label\MYoldlabel
}


% {{{ bibliography }}}

% add section for references to table of contents
\newcommand{\addreferencesection}{
  \phantomsection
  \addcontentsline{toc}{section}{References}
}


% {{{ mathabbreviations }}}

\newcommand{\la}{\leftarrow}
\newcommand{\sse}{\subseteq}
\newcommand{\ra}{\rightarrow}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\eset}{\emptyset}


% {{{ paragraphperiod }}}


\let\origparagraph\paragraph
\renewcommand{\paragraph}[1]{\origparagraph{#1.}}


% {{{ allowdisplaybreaks }}}
% allows page breaks in large display math formulas

\allowdisplaybreaks


% {{{ sloppy }}}
% avoid math spilling on margin

\sloppy

% {{{ complexityclasses }}}

\newcommand{\cclassmacro}[1]{\texorpdfstring{\textbf{#1}}{#1}\xspace}
\newcommand{\p}{\cclassmacro{P}}
\newcommand{\np}{\cclassmacro{NP}}
\newcommand{\subexp}{\cclassmacro{SUBEXP}}

% {{{ paralist }}}

\usepackage{paralist}

% {{{ comment }}}

\usepackage{comment}


%{{{Bra Ket Notation}}}
\usepackage{braket}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../planted"
%%% End:

